RTLola on Board: Testing Real Driving Emissions on your Phone

This paper is about shipping runtime verification to the masses. It presents the crucial technology enabling everyday car owners to monitor the behaviour of their cars in-the-wild. Concretely, we present an Android app that deploys RTLola runtime monitors for the purpose of diagnosing automotive exhaust emissions. For this, it harvests the availability of cheap bluetooth adapters to the On-Board-Diagnostics (OBD) ports, which are ubiquitous in cars nowadays. We detail its use in the context of Real Driving Emissions (RDE) tests and report on sample runs that helped identify violations of the regulatory framework currently valid in the European Union.

==> author_comments.tex <==
% Version 1.1
% (c) Pedro D'Argenio, Sebastian Biewer



\newif\ifcomments
\newif\ifshowremoved

\usepackage{xcolor}
\usepackage[absolute]{textpos}
\usepackage{everypage}

\definecolor{lightblue}{RGB}{210,210,225}
\definecolor{lightred}{RGB}{225,210,210}
\definecolor{lightgreen}{RGB}{210,225,210}
\definecolor{lightyellow}{RGB}{225,222,200}
\definecolor{lightpurple}{RGB}{225,210,225}
\definecolor{warningyellow}{RGB}{247, 245, 187}
\definecolor{darkergreen}{RGB}{0,64,0}
\definecolor{darkred}{RGB}{128,0,0}
\definecolor{darkblue}{RGB}{0,0,139}
\definecolor{darkgreen}{RGB}{0,128,0}
\definecolor{darkpurple}{RGB}{128,0,128}
\definecolor{warningorange}{RGB}{124, 81, 0}
\definecolor{eyecancerpink}{rgb}{1.0, 0.0, 1.0}
\definecolor{radiationyellow}{rgb}{0.8, 1.0, 0.0}

\newcommand{\colorpar}[3]{\colorbox{#1}{\parbox{#2}{#3}}}

%% \newcommand{\marginremark}[2]{\marginpar{\color{#1}{#2}}}
\newcommand{\marginremark}[4]{\marginpar{\colorpar{#2}{\linewidth}{\color{#1}\tiny{[#3]~ #4}}}}

\newcommand{\citeref}[2]{\href{#1}{#2}~\cite{#1}}

\def\enablecomments{
  \commentstrue
  \enableheader
}

\def\enableheader{
\AddEverypageHook{{
\begin{textblock*}{\paperwidth}(0mm,2mm) {
%\begin{center}
\centering
\textcolor{gray}{\textbf{
\Huge! D R A F T !
}\\\vspace*{1mm}
\footnotesize
%Disable author comments to remove this watermark.
}
%\end{center}
}
\end{textblock*}
}}\par
\AddEverypageHook{{
\begin{textblock*}{\paperwidth}(0mm,9mm) {
%\begin{center}
\centering
\textcolor{gray}{
\footnotesize
Disable author comments to remove this watermark.
}\\
%\end{center}
}
\end{textblock*}
}}\par
}

\makeatletter
\def\THICKhrulefill{\leavevmode \leaders \hrule height 5pt\hfill \kern \z@}
\makeatother
\newcommand{\highlightedremark}[4]{%
  \begin{center}\fcolorbox{#1}{#2}{%
  \begin{minipage}{.98\linewidth}\color{#1}%
  \textbf{\THICKhrulefill[ #3 ]\THICKhrulefill}%
  \par\noindent#4\end{minipage}}\end{center}%
}

\newcommand{\remarkHH}[1]{\ifcomments\marginremark{eyecancerpink}{radiationyellow}{HH}{#1}\fi}
\newcommand{\remarkPRD}[1]{\ifcomments\marginremark{darkred}{lightred}{PRD}{#1}\fi}
\newcommand{\remarkSB}[1]{\ifcomments\marginremark{darkergreen}{lightgreen}{SB}{#1}\fi}
\newcommand{\remarkMK}[1]{\ifcomments\marginremark{darkpurple}{lightpurple}{MK}{#1}\fi}
\newcommand{\remarkYS}[1]{\ifcomments\marginremark{darkblue}{lightblue}{YS}{#1}\fi}
\newcommand{\remarkMS}[1]{\ifcomments\marginremark{darkblue}{lightblue}{MS}{#1}\fi}

\newcommand{\hrmkSB}[1]{\ifcomments\highlightedremark{darkergreen}{lightgreen}{SB}{#1}\fi}
\newcommand{\hrmkHH}[1]{\ifcomments\highlightedremark{eyecancerpink}{radiationyellow}{HH}{#1}\fi}
\newcommand{\hrmkPRD}[1]{\ifcomments\highlightedremark{darkred}{lightred}{PRD}{#1}\fi}
\newcommand{\hrmkMK}[1]{\ifcomments\highlightedremark{darkpurple}{lightpurple}{MK}{#1}\fi}
\newcommand{\hrmkMS}[1]{\ifcomments\highlightedremark{darkblue}{lightblue}{MS}{#1}\fi}
\newcommand{\hrmkYS}[1]{\ifcomments\highlightedremark{darkblue}{lightblue}{YS}{#1}\fi}
\newcommand{\removed}[1]{\ifcomments\highlightedremark{warningorange}{warningyellow}{REMOVED CONTENT}{\ifshowremoved #1 \else Add ``showremovedtrue'' below ``commentstrue'' to display removed content. \fi}\fi}

==> platform.tex <==
Worldwide over one billion cars are in use~\cite{cars-worldwide}, generating an immense amount of real-world driving data.
The \emph{Portable Car Data Platform} (\pcdp) provides a way to harvest this data by specifying a format for collection, analysis, and exchange of this data.
\APP is fully compatible with \pcdp and can thus upload any collected data.
This allows for conducting any further analysis after the fact.
As an example, the data presented in \Cref{tbl:tests} is an aggregation of the \rde drives runs mentioned in \Cref{sec:rde}.
The platform is not limited to data from cars with internal-combustion engines; by design, it is compatible with other engine kinds like electrical engines as well.

%For example, after donating the trip data of the two RDE tests in section~\ref{sec:rde}, we could identify that the second trip violated RDE conditions because the driving behaviour was too aggressive regarding accelerations.  %% MS: Makes no sense since the app is already capable of doing so...

\begin{table}[t]
\centering
\begin{tabular}{ l c c c @{\hskip .5cm} c c c }
 & \multicolumn{3}{c}{Drive 1} & \multicolumn{3}{c}{Drive 2} \\
  \cmidrule(r{.4cm}){2-4} \cmidrule(l{-.1cm}){5-7}
 & \makecell[cc]{Distance \\$\left[\SI{}{\kilo\meter}\right]$} & \makecell[cc]{\textit{\NOx} \\ $\left[\SI[per-mode=symbol]{}{\milli\gram\per\kilo\meter}\right]$} & \makecell[cc]{\textit{\COx} \\ $\left[\SI[per-mode=symbol]{}{\gram\per\kilo\meter}\right]$} & \makecell[cc]{Distance \\ $\left[\SI{}{\kilo\meter}\right]$} & \makecell[cc]{\textit{\NOx} \\ $\left[\SI[per-mode=symbol]{}{\milli\gram\per\kilo\meter}\right]$} & \makecell[cc]{\textit{\COx} \\ $\left[\SI[per-mode=symbol]{}{\gram\per\kilo\meter}\right]$} \\
 \midrule
Urban & 35.45 & 137 & 222 & 37.46 & 102 & 251 \\
Rural & 22.33 & 305 & 154 & 27.40 & 90 & 172 \\
Motorway & 26.10 & 241 & 153 & 25.37 & 105 & 175 \\
Total  & 83.88 & 214 & 183 & 90.22 & 99 & 105 \\
    \end{tabular}
    \vspace{.3cm}
    \caption{Aggregation of the emission data based on the \pcdp.}
    \label{tbl:tests}
\end{table}

%Based on the \pcdp, we aim to build a data set enabling insights not only into real-world emissions of vehicles with internal combustion engines.
%With the advent of electric vehicles other questions become pressing, for instance, how long do the batteries of an electric car actually last under real-world conditions.
%Similar to the emissions scandal, manufacturers may try to tweak there numbers for newer forms of transportation.\remarkMS{I find it questionable to accuse manufacturers of deliberate deception precautionary --- of course we should limit their options, I just recommend a less accusatory tone of voice.}

\pcdp builds upon the \emph{Portable Car Data Format} (\pcdf), a format specified in \textsc{json} schema\footnote{\url{https://json-schema.org/}}.
A \pcdf file contains recorded and timestamped events such as an \obd response, including its payload in raw bytes.
For data processing, the payload is parsed, making data points such as the current velocity of the car readily available.
The difference of representation is captured in the two variants of \pcdf: \emph{persistent} \pcdf (\ppcdf) and \emph{intermediate} \pcdf (\ipcdf).

The persistent format is intended for long term storage and transmission.
Encoding utilizes MessagePack\footnote{\url{https://msgpack.org/}} to achieve greater space efficiency in binary form.
In comparison, the purpose of iPCDF the exchange of collected data for further analysis.
Its strong ties to the \textsc{json} format enables various tools of parsing the format without further ado.

A conversion tool for converting \ppcdf into \ipcdf and vice versa is available.\remarkMS{Could anyone provide a link?}
Our tool implements a large part of the OBD standard allowing tools to directly retrieve the information they need from an iPCDF file without having to implement the standard themselves.
\remarkMS{Could anyone clarify the sentence abolve? What standard?  Which tool --- conversion or the app?  I thought the conversion tool only converts \ppcdf/\ipcdf?}


%The \emph{Portable Car Data Format} (PCDF) is a standardized\remarkSB{it is standardised by us, this should be mentioned} format specified in JSON schema\footnote{\url{https://json-schema.org/}}\remarkMS{We should be extremely careful here: standardization requires that \emph{several parties} agree upon a common format.  This is \textbf{not} the case here. This is deliberate deception.}.
%A PCDF file contains recorded events which are timestamped and carry additional information.
%For instance, OBD responses of the car are captured as events containing the raw bytes returned by the car.
%For processing, one needs to parse the actual information, such as the engine's RPM or the current velocity, out of the bytes.
%To this end, there are two variants of PCDF, \emph{persistent} PCDF (pPCDF) and \emph{intermediate} PCDF (iPCDF).

%The persistent format is intended for long term storage and transmission over the internet.
%It relies on MessagePack\footnote{\url{https://msgpack.org/}} for encoding the JSON structures in a more space efficient binary form.
%In addition, a pPCDF file only contains the minimal necessary information such as the raw bytes of an OBD response.
%In comparison, iPCDF is intended for exchanging collected data for further analysis.
%It is JSON-based so that it is easy to parse by various tools.
%We provide a conversion tool for converting between pPCDF and iPCDF.
%Events of an iPCDF file may carry additional information such as parsed OBD data.
%Our tool implements a large part of the OBD standard allowing tools to directly retrieve the information they need from an iPCDF file without having to implement the standard themselves.

\hrmkMS{I struggle to fully understand the following paragraph(s).  What kind of aggregations take place on the app?  The \rtlola aggregations?  Also, you mentioned above (see code comment) that a \ppcdf file contains raw data from \emph{an} \obd response.  Here, it sounds more like a \ppcdf file summarizes an entire execution?  Also, \rtlola does not support the \ipcdf format, so the app extracts the information inside the message rather than the \ipcdf message itself.}
The \APP allows collecting data from various sources such as OBD but also, for example, the phone's internal GPS module.
It aggregates all this information in a pPCDF file which can then be uploaded and used for further offline analysis.
In addition, it provides a live stream of the events in iPCDF form.
The live stream is used to update the UI of the app as well as to hand over the events to \rtlola to perform online monitoring.
\rtlola is the perfect match for PCDF as it allows to process streams of timed events efficiently and with memory guarantees.

Based on this infrastructure, we envision further analysis tools to emerge, \ie, a web interface for interactively exploring and evaluating car related data providing valuable insights into on-the-road emissions and more.
The \APP is at the heart of that infrastructure allowing laypersons to collect and contribute data. 
\hrmkMS{It feels strange to me to emphasize that we have platform and expect others to provide an interactive web interface, data, and analysis tools.  We should place the contribution in the foreground, not action items for readers that may or may not be picked up eventually.}

% \begin{itemize}

%     \item we store many kinds of important car / trip related data (e.g. OBD, GPS, External Sensors) uniformly in one place
%     \item formats are event based and json schema specified (fits the idea of event based \textbf{RTLola-Inputstreams}), json is easy to parse
%     \item we introduce two types of PCDF : persistent and intermediate, p for memory efficient saving and i for data analysis
%     \item we offer a tool to easily convert p in i and vice versa, containing a big part of the OBD standard, we use this to translate the messages received via the OBD interface of the car
%     \item The app offers a tracking interface in which the user can select PIDs, i.e. measured values that he wants to track, these are logged in PCDF format.
%     \item These stored tracks can then be converted to iPCDF format and used for analysis and presentation of the data. Within the app it is possible to review past tracks event by event and view visualizations like the speed-time diagram.
%     \item we offer the possibilty to upload trip data to our server for further analysis\\
%     \remarkYS{maybe insert pictures of an OBD pPCDF and iPCDF Event}
%     \item [Future Work] we plan to offer an online interface where users can upload their PCDF Trip data and perform data analysis
    
% \end{itemize}

%\paragraph{Lola for Android.} Here we can explain that the RDE specification can be replaced by, e.g., EV specifications, and that Lola could be ripped out of the app to be used in a competely different app/context.







==> preliminaries.tex <==
In 2015, the Diesel Emissions Scandal unveiled an uncomfortable truth about the work of many passenger car manufacturers. 
Millions of diesel powered cars were equipped with tampered emission cleaning systems; during official test situations they performed commendable, but in real driving situations they polluted the environment most of the time.  
Among the early discoveries and most severe cases is Volkswagen. 
Their cars were equipped with engine control units provably containing software components to detect whether the car is undergoing an official emissions test according to the, then effective, admission regulations. 
These regulations define a driving cycle called \emph{New European Driving Cycle} (NEDC) with the weakness of enforcing tests with a constructed and very unnatural driving behaviour largely containing constant speed phases and repeating patterns---it can be detected easily. 

Research and the vehicle regulations consortium have been taking up these weaknesses
 to suggest solutions. 
A product of research is a breach of
the (proprietary) software running in Volkswagen cars, which gained valuable insights into their defeat devices~\cite{domke}. 
These devices were so precise that even small deviations from the NEDC caused a significant increase of regulated emissions. 
Small input deviations lead to large output deviations---this observation was taken up by D'Argenio et al.~\cite{DBLP:conf/esop/DArgenioBBFH17} and baked into a set of formal definitions for \emph{clean} behaviour of systems. 
Systems that are not clean would be called \emph{doped}, and the usage of defeat devices in diesel cars becomes an instance of \emph{software doping}. 
The theory allows model-checking~\cite{allReactPapersRelated} and testing, and has been successfully used to find cases of software doping in practice~\cite{DBLP:conf/qest/BiewerDH19,TOMACS,Dimitrova}.
The official homologation process has been adapted to better cover real driving behaviour; 
the NEDC has been replaced by the \emph{Worldwide Harmonised Light Vehicles Test Cycle} (WLTC), which eliminates constant speed phases and pattern repetition, and represents a more dynamic driving behaviour.
In addition, a relatively large set of driving cycles is considered for \emph{Real Driving Emissions} (RDE) tests on the road  under presumably realistic conditions.
%To rectify the problems with earlier regulations, the EU specified the \emph{Real Driving Emissions} (RDE) test procedure.
%The RDE test procedure dose not share the problematic characteristics of earlier test procedures in that RDE tests are conducted on-the-road under presumably realistic conditions.
The RDE regulation specifies broad certification conditions for tests conducted under real-word conditions, on public roads and during working days.
An (informal) specification document~\cite{LEX:32017R1151} spells out precise preconditions a trip, \ie, a trajectory driven with a car, has to satisfy in order to count as a valid RDE test.
These preconditions include constraints on the route, allowed altitudes and speeds, and on the dynamics of the driving profile. An RDE test must traverse three phases, the urban, the rural, and the motorway phase covering different speed ranges and each making up approximately one third of the total trip distance.
Table~\ref{tbl:rde} provides an overview of the constraints for all three phases.
%
\begin{table}[t]
    \centering
    \def\arraystretch{1.2}
    \small
    \begin{tabular}{|p{.25\textwidth}|p{.21\textwidth}|p{.21\textwidth}|p{.2\textwidth}|}
    \hline
    & Urban & Rural & Motorway \\ \hline
    Ratio Range [\%] & $[29,44]$ & $[23,43]$ & $[23,43]$ \\ \hline
    Speed Range [km/h] & $[0, 60]$ & $]60, 90]$ & $]90, 160]$ \\ \hline
    Distance [km] & $\geq16$ & $\geq16$ & $\geq16$ \\ \hline
    \raggedright Additional Constraints & \raggedright  stop percentage between 6\% and 30\% of urban time; average velocity in range $[15,40]$km/h &  & $>100$km/h for at least 5mins \\ \hline
    \raggedright Temperature [K] & \multicolumn{3}{p{.66\textwidth}|}{\centering moderate: $[273,303]$; extended: $[266,273[$ or $]303,308]$ } \\ \hline
    \raggedright Altitude [m] & \multicolumn{3}{p{.66\textwidth}|}{\centering moderate: $<700$; extended: $]700,1300]$ } \\ \hline
    \raggedright Speed Limit [km/h] & \multicolumn{3}{p{.66\textwidth}|}{\centering 145 (]145,160] for at most 3\% of motorway time)} \\ \hline
    \end{tabular}
    \vspace{3mm}
    \caption{Some constraints for the three phases of RDE tests \cite{hermanns:2018:verification}.}
    \label{tbl:rde}
\end{table}


In an official RDE test, a calibrated \emph{portable emissions measurement system} (PEMS) is connected to the car's exhaust pipe and to the OBD interface. It  measures the amount of several gases and particles emitted by the car, and combines this information with the information received from the OBD interface. The costs for a PEMS are in the order of approx. \euro{250,000}, which is prohibitive for individuals (as well as researchers).
Nevertheless, without a PEMS it is still possible to access the OBD interface, which is documented in the official regulation.
The amount of data offered through OBD depends on the type of engine, emission cleaning system and other components of the car.
There are several minimal combinations of OBD data which can be combined to get a good approximation of emitted gases.
Köhl et al. successfully performed RDE tests solely using OBD data showing a violation with an Audi A7~\cite{DBLP:conf/rv/KohlHB18}.
\remarkMK{We should make explicit somewhere that these are not genuine RDE tests but rather a lightweight best-effort version of RDE tests.}
One of their major contributions is a formalisation of the informal RDE specification in the official regulation.
They use the monitoring framework StreamLAB, and specify RDE trips in a variant of StreamLAB's specification language RTLola~\cite{lola}.
\remarkMK{We used Lola 2.0 with discrete windows for that not RTLola.}
\hrmkSB{ToDo: Lola}
Prior to this work, StreamLAB was able to do monitoring on personal computers and Field Programmable Gate Arrays (FPGAs).
Other verification tools, for example APHzip~\cite{aphzip,maybeMore}, have been ported to mobile devices (such as mobile phones and tablets).





